On the Expressiveness of Intensional Communication

The expressiveness of communication primitives has been explored in a common framework based on the pi-calculus by considering four features: synchronism (asynchronous vs synchronous), arity (monadic vs polyadic data), communication medium (shared dataspaces vs channel-based), and pattern-matching (binding to a name vs testing name equality). Here pattern-matching is generalised to account for terms with internal structure such as in recent calculi like Spi calculi, Concurrent Pattern Calculus and Psi calculi. This paper explores intensionality upon terms, in particular communication primitives that can match upon both names and structures. By means of possibility/impossibility of encodings, this paper shows that intensionality alone can encode synchronism, arity, communication-medium, and pattern-matching, yet no combination of these without intensionality can encode any intensional language.

==> eptcsdata.tex <==
\providecommand{\firstpage}{30}
\providecommand{\publicationstatus}{J. Borgstr\"om, S. Crafa (Eds.): Combined Workshop on Expressiveness in\\ Concurrency and Structural Operational Semantics (EXPRESS/SOS 2014)\\
EPTCS 160, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.160.4}{10.4204/EPTCS.160.4}}

